Meta-SysId: A Meta-Learning Approach for Simultaneous Identification and Prediction

In this paper, we propose Meta-SysId, a meta-learning approach to model sets of systems that have behavior governed by common but unknown laws and that differentiate themselves by their context. Inspired by classical modeling-and-identification approaches, Meta-SysId learns to represent the common law through shared parameters and relies on online optimization to compute system-specific context. Compared to optimization-based meta-learning methods, the separation between class parameters and context variables reduces the computational burden while allowing batch computations and a simple training scheme. We test Meta-SysId on polynomial regression, time-series prediction, model-based control, and real-world traffic prediction domains, empirically finding it outperforms or is competitive with meta-learning baselines.

==> check_list.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
  \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{}. We will publicize the code after the decision.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> figs/target-position-drone.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: 
\path (0,150); %set diagram left start at 0, and has height of 300

%Shape: Axis 2D [id:dp016311997038469972] 
\draw  (68,261.6) -- (102,261.6)(71.4,231) -- (71.4,265) (95,256.6) -- (102,261.6) -- (95,266.6) (66.4,238) -- (71.4,231) -- (76.4,238)  ;
%Image [id:dp63310098461719] 
\draw (173.37,188.61) node [rotate=-329.82] {\includegraphics[width=68.91pt,height=19.2pt]{figs/free-drone-icon-1.jpg}};
%Image [id:dp4962188933591156] 
\draw (84.3,127.34) node  {\includegraphics[width=31.95pt,height=30.51pt]{figs/wind (2).png}};
%Straight Lines [id:da004825037712003155] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (72.6,139) -- (102.48,109.12) ;
\draw [shift={(104.6,107)}, rotate = 135] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Shape: Star [id:dp0010117365438584436] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (101.8,189) -- (103.5,192.87) -- (107.32,193.49) -- (104.56,196.5) -- (105.21,200.76) -- (101.8,198.75) -- (98.39,200.76) -- (99.04,196.5) -- (96.28,193.49) -- (100.1,192.87) -- cycle ;
%Curve Lines [id:da051134682140536736] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (103.6,198) .. controls (174.6,229) and (177.6,215) .. (171.6,191) ;
%Image [id:dp3571103369908555] 
\draw (161.3,127) node  {\includegraphics[width=37.95pt,height=22.5pt]{figs/mexican-hat.png}};

% Text Node
\draw (102,261.4) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (54,220.4) node [anchor=north west][inner sep=0.75pt]    {$y$};
% Text Node
\draw (67,145) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{lmr}\selectfont \textcolor[rgb]{0.29,0.56,0.89}{wind}}};
% Text Node
\draw (82,208) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{lmr}\selectfont target}\\{\fontfamily{lmr}\selectfont position}};
% Text Node
\draw (159,220) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {\textcolor[rgb]{0.82,0.01,0.11}{{\fontfamily{lmr}\selectfont actual}}\\\textcolor[rgb]{0.82,0.01,0.11}{{\fontfamily{lmr}\selectfont trajectory}}};
% Text Node
\draw (114,124) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textcolor[rgb]{0.29,0.56,0.89}{=}};


\end{tikzpicture}

==> figs/trajectory-tracking-drone.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Axis 2D [id:dp016311997038469972] 
\draw  (68,261.6) -- (102,261.6)(71.4,231) -- (71.4,265) (95,256.6) -- (102,261.6) -- (95,266.6) (66.4,238) -- (71.4,231) -- (76.4,238)  ;
%Image [id:dp63310098461719] 
\draw (183.37,160.61) node [rotate=-329.82] {\includegraphics[width=68.91pt,height=19.2pt]{figs/free-drone-icon-1.jpg}};
%Curve Lines [id:da7540138277924193] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}]  (122.44,237.36) .. controls (183.57,244.27) and (182.38,187.61) .. (167.6,162) ;
\draw [shift={(119.6,237)}, rotate = 8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Curve Lines [id:da5363478495282654] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] [dash pattern={on 3.75pt off 3pt on 7.5pt off 1.5pt}]  (168.6,163) .. controls (145.32,136.81) and (157.79,113.44) .. (162.25,96.25) ;
\draw [shift={(166.6,89)}, rotate = 120.96] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Curve Lines [id:da42465085473086406] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (118.6,237) .. controls (231.6,249) and (190.6,183) .. (184.6,159) ;
%Image [id:dp4962188933591156] 
\draw (84.3,127.34) node  {\includegraphics[width=31.95pt,height=30.51pt]{figs/wind (2).png}};

% Text Node
\draw (102,261.4) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (54,220.4) node [anchor=north west][inner sep=0.75pt]    {$y$};
% Text Node
\draw (92,184) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{lmr}\selectfont reference}\\{\fontfamily{lmr}\selectfont trajectory}};
% Text Node
\draw (202,199) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {\textcolor[rgb]{0.82,0.01,0.11}{{\fontfamily{lmr}\selectfont actual}}\\\textcolor[rgb]{0.82,0.01,0.11}{{\fontfamily{lmr}\selectfont trajectory}}};
% Text Node
\draw (67,145) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\fontfamily{lmr}\selectfont \textcolor[rgb]{0.29,0.56,0.89}{wind}}};


\end{tikzpicture}

==> sections/01_introduction.tex <==
Identifying the system parameters from the input and responses of the system, which is also known as system identification, is the cornerstone of system modeling. Classically, the system identification is done by solving the optimization problem, which minimizes the discrepancy between the model-predicted and observed responses with respect to the model class. Even though such optimization-based approaches are the de facto standard methods for system identification, they have two major drawbacks: (1) they assume to know a proper model class, and (2) the optimization problem can be ill-conditioned as the inverse nature of the problem (e.g., the number of data points must be larger than the number of system parameters).

% For instance, the learned classifier trained to discriminate cats from dogs quickly adapts to classify horse from cats and dogs with small amount of horse images.

\textcolor{red}{Some sentence is missing to link the sys. id and Meta-learning.}
Meta-learning is a collection of learning algorithms that learn to adapt to new tasks quickly with a handful of data. Depending on the adaptation mechanism, the meta-learning algorithms are generally categorized as optimization-based and black-box methods. The optimization-based method adapts to new tasks by optimizing the network parameters while the black-box method utilizes an encoding network to infer the new task. Although the optimization-based methods often outperform the black-box methods, they typically come at the cost of the second-order optimization during the meta-training.

We interpret the adaptation of the optimization-based meta-learning as the identification of the system from the observational data. Based on this interpretation, we propose Meta-Id that learns to identify the system parameters and select the model class jointly. We cast the training problem of Meta-Id as a bi-level optimization, where the inner optimization is for identifying the systems and the outer optimization is for learning the function class of the systems. In other words, Meta-Id is an optimization-based meta-learning method, which adapts to the specific task by solving the system identification. As an optimization-based meta learning, training Meta-Id involves solving the bi-level optimization, which requires second-order derivatives. We overcome this difficulty by employing a training trick inspired by the target network \cite{lillicrap2015continuous}. The target-network trick allows us to train Meta-Id with plain gradient descent methods while being network-architecture agnostic. Additionally, we observe that it serves as a noise regularization so that the trained Meta-Id well generalizes.

To validate Meta-Id, we apply it to solve the static function regression, time-series prediction, and control problems, all of which has unknown system parameters. Using the experimental results, we show that Meta-Id outperforms the optimization-based and black-box meta-learning baselines. Furthermore, we confirm that Meta-Id overcomes the drawbacks of the classical parameter identification by combining the idea of meta-learning into the framework of system identification. 

% From the experimental results, we confirm that Meta-Id overcomes the drawbacks of the classical parameter identification by combining the idea of meta-learning to the framework of system identification. 












==> sections/01_introduction_jkp.tex <==
\label{section:intro}

To predict responses of a complicated real-world system, it is common to first specify a model class, then use real-world data to identify model parameters. Though this \textit{modeling and system identification} paradigm has enabled remarkable scientific advances, it has many drawbacks. For example, assuming incorrect knowledge of model class can lead to model misspecification. Even with the correct model class, parameter identification can be ill-conditioned if the dataset size is too small. 
Many recent approaches combine modeling and system identification by defining overly flexible model classes (e.g. black-box neural networks) and relying on large datasets for model-fitting. 
These approaches have been able to model complex systems that are beyond human conception, revolutionizing scientific discovery \cite{jumper2021highly, brunton2016discovering, degrave2022magnetic, kochkov2021machine}. 

Despite the empirical success of these black-box approaches, they have shown limited generalization capability, especially to changing system parameters. One possible approach to address generalization issues is to combine flexible models with data from sets of related systems. In this study, we aim to model sets of systems whose behaviors are governed by common but unknown laws and where individual systems are differentiated by their context. 
%These assumptions are general enough so that most engineering and natural systems belong to this category. 
We propose \ourmethod, a meta-learning method to model the target system. Inspired by the ``modeling and identification" framework, \ourmethod{} considers target systems in the form of $y=f_{\theta}(x, c)$, where $\theta$ denotes the function class shared by the target systems, and $c$ denotes system-specific context characteristics. \ourmethod{} learns the function class $f_\theta$ from data during the meta-training (i.e., learning $f_\theta$) and performs system identification online to find the proper system-specific context $c$.

% How \ourmethod{} works. 


% Strong point and novelty
This separation between model parameters $\theta$ and context variables $c$ provides two major advantages over other optimization-based meta-learning algorithms (e.g., \cite{finn2017model,nichol2018first}). First, during testing, this separation reduces the burden of adaptive mechanisms, which only optimize for task-specific context $c$ while fixing class parameters $\theta$. In addition, this separation allows us to employ a training trick based on the exponential moving average (EMA), enabling us to train \ourmethod{} with gradient descent methods, and critically without computing second-order gradients. The contributions of this work are summarized as follows:
\begin{itemize}[leftmargin=0.5cm]
\vspace{-0.25cm}
    \item We propose \ourmethod, a meta-learning approach that enjoys strong empirical performance, model-agnosticism, and interpretable behavior when modeling various systems.
    \item We propose a simple yet effective training trick for \ourmethod{} that overcomes the burden of second-order derivative calculations while regularizing against noise.
    \item We empirically demonstrate that our approach is competitive to or outperforms various meta-learning baselines in static function regression, time-series prediction, offline model-based control domains. %, and real-world traffic flow prediction .
\end{itemize}


==> sections/01_introduction_new.tex <==
% Meta-learning -> optimization-based/black-box depending on the adaptation mechanism-> the optimization-based methods explicitly solve optimization problem as the adaptation

% However, 
The ability to quickly learn (or adapt) to new scenarios is one of the critical properties that natural intelligence makes thrive. Implementing such capability in artificial intelligence has been explored in the name of Meta-learning, a collection of learning algorithms that learn to adapt to new tasks quickly with a handful of data.

Meta-learning algorithms are generally categorized as \textit{optimization-based} and \textit{black-box methods} depending on the adaptation mechanism. The optimization-based methods \cite{finn2017model, nichol2018first} adapt to new tasks by conducting explicit optimizations on the network parameters $\theta$ to form the task-adapted parameters $\theta'$ during adaptation. The black-box methods \cite{mishra2018simple, garnelo2018conditional, gordon2019convolutional, kim2019attentive} learn the (task) inference network and produce a task embedding $c$ as adaptation to perform the task with $\theta$ (i.e., $\theta'=\{\theta, c\}$). Often, the optimization-based methods outperform the black-box methods by enjoying model-agnosticism and a positive inductive bias from explicit optimizations. However, they typically come at the cost of the second-order optimization during the meta-training. \textcolor{red}{The black-box methods decompose the role of $\theta$ and $c$ by its construction; thus, they often show interpretable behavior to the change of $c$. However, they show relatively weak performances than the optimization-based methods.}

\textcolor{red}{Need to clearly state our target problems so that later the reviewers wouldn't mention about the image-based meta learning tasks.}

In this paper, we propose Meta-Id, a meta-learning algorithm that bridges the optimization-based and black-box methods and is inspired by system identification (SysId). Specifically, Meta-Id explicitly solves the optimization problem of SysId, as the optimization-based method, and finds the task context $c$. It then utilizes the identified $c$ and $\theta$ to perform the downstream task, as the black-box method. We cast the training problem of Meta-Id as a bi-level optimization, where the inner optimization is for identifying the context and the outer optimization is for learning the model parameter. Solving the bi-level optimization can be done, as in the majority of optimization-based meta-learning methods, entails calculating the second-order derivatives, which degrades the train-ability (i.e., of wall-clock time and memory consumption of training) and stability of algorithm \cite{antoniou2018train, ye2021train}. We overcome this difficulty by employing a training trick inspired by the target network \cite{lillicrap2015continuous}. The target-network trick allows us to train Meta-Id with plain gradient descent methods while being network-architecture agnostic. Additionally, we observe that it serves as a noise regularization to improve the generalization of our approach. 

We validate Meta-Id on the following learning problems: solving the static function regression, time-series prediction, and online control, all of which have unknown system parameters. From the experimental results, we demonstrate that Meta-Id outperforms the optimization-based and black-box meta-learning baselines. \textcolor{red}{Furthermore, we apply Meta-Id to predict time-series collected from the real-world traffic systems where the meaning of context is not evinced. From the results, we also confirm Meta-Id still provides performance gain by levering the adaptation procedure to the \textit{virtual} context.}  We summarize our contributions as follows:
\begin{itemize}[leftmargin=0.5cm]
\vspace{-0.25cm}
    \item  We propose a new meta-learning approach hybridizing the optimization-based and block-box methods 
    while enjoying the strong empirical performance, model-agnosticism, as well as interpretable behavior of $\theta$ and $c$.
    \item We overcome the burden of second-order derivative calculations via a simple-yet-effective training trick for Meta-Id that also serves as a noise regularizer.
    \item We empirically demonstrate that our approach outperforms baseline optimization-based and black-box meta-learning methods in various domains, including synthetic and \textcolor{red}{real-world datasets.}
\end{itemize}
\vspace{-0.25cm}

% To summarize our contributions are:





% We interpret the adaptation of the optimization-based meta-learning as the identification of the system from the observational data. Based on this interpretation, we propose Meta-Id that learns to identify the system parameters and select the model class jointly. We cast the training problem of Meta-Id as a bi-level optimization, where the inner optimization is for identifying the systems and the outer optimization is for learning the function class of the systems. In other words, Meta-Id is an optimization-based meta-learning method, which adapts to the specific task by solving the system identification. 

% As an optimization-based meta learning, training Meta-Id involves solving the bi-level optimization, which requires second-order derivatives. We overcome this difficulty by employing a training trick inspired by the target network \cite{lillicrap2015continuous}. The target-network trick allows us to train Meta-Id with plain gradient descent methods while being network-architecture agnostic. Additionally, we observe that it serves as a noise regularization so that the trained Meta-Id well generalizes.



==> sections/02_related.tex <==

\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
         \includegraphics[width=\textwidth]{main_cand/catchy_blackbox.pdf}
         \caption{Black-box meta-learning}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
         \includegraphics[width=\textwidth]{main_cand/catchy_opt.pdf}
         \caption{Optimization-based meta-learning}
     \end{subfigure}
     \hfill
          \begin{subfigure}[b]{0.325\textwidth}
         \centering
         \includegraphics[width=\textwidth]{main_cand/catchy_metasysid.pdf}
         \caption{\ourmethod{}}
     \end{subfigure}
    \caption{\footnotesize Differences in meta--training and meta--testing between meta-learning model types. (a) Black--box models obtain context information via state encoders. (b) Optimization--based models do not explicitly divide state and context information, but optimize of all model parameters online. (c) \ourmethod{} obtains context information by solving an optimization problem.}
    \label{fig:catchy}
\end{figure}


\paragraph{Learning to adapt} Learning models for task adaptation has been investigated under many names, some of which include meta-learning \cite{ravi2016optimization, finn2017model, nichol2018first, mishra2018simple, rusu2018meta, santoro2016meta}, online system identification \cite{fu2016one, yu2017preparing, richards2021adaptive, chen2021context, ball2021augmented, lee2020context}, and neural processes (NP) \cite{garnelo2018conditional, gordon2019convolutional, kim2019attentive}. Adaptation methods for regression can be classified as \emph{optimization-based} (e.g., MAML \cite{finn2017model}, Reptile \cite{nichol2018first}) or \emph{black-box}  (e.g., MANN \cite{santoro2016meta}, SNAIL\cite{mishra2018simple}, NP) methods depending on whether they perform online optimization to find the task-adapted model parameters or employ a meta-learned adaptation method to infer task-specific context. Optimization-based method often show stronger empirical performance, but come at the cost of higher computational time, more memory consumption, and training instabilities \cite{antoniou2018train, ye2021train}. Black-box methods are often faster and easier to train, but their adaptation capability can be limited by the learning model's representation capacity. 

\ourmethod{} shares a similarity to black-box methods as it learns a context online to perform downstream tasks. However, \ourmethod{} can be seen as an optimization-based method as it perform online optimization to find that context. Unlike MAML and Reptile, which adapt model parameters, \ourmethod{} optimizes to find the best context as an input to the model. This algorithmic choice allows it to be efficiently trained and evaluated in batch.

\paragraph{Solving bi-level optimizations to learn} Casting adaptation as a bi-level optimization problem can be found in various applications \cite{amos2017optnet, amos2017input, rajeswaran2019meta, rubanova2021constraint, finn2017model, nichol2018first, lee2019meta, bertinetto2018meta}. Solving bi-level optimizations to train a model roughly categorized into methods that (1) formulate the inner optimization so that it has a closed-form solution \cite{lee2019meta, bertinetto2018meta}, (2) differentiate the argmin via implicit differentiation \cite{amos2017optnet, amos2017input, rajeswaran2019meta}, and (3) backpropagate through the inner optimization step \cite{rubanova2021constraint, finn2017model}. 
The first two methods limit the model class into a certain family to estimate the gradient without bias \cite{blondel2021efficient, liao2018reviving}, while the third method entails intensive memory usage during training and possibly biases the solution of the inner-level optimization. 
The EMA trick we employ to train \ourmethod{} circumvents all of these shortcomings, letting us keep flexible model classes (and model agnosticism) while avoiding backpropagating through the inner optimization steps.



==> sections/05_1_polynomial.tex <==
\begin{figure}[t]
   \begin{minipage}{0.65\textwidth}
     \centering
     \includegraphics[width=.90\linewidth]{figs/poly_overall.pdf}
     \caption{Polynomial prediction}
     \label{fig:poly_overall}
   \end{minipage}\hfill
   \begin{minipage}{0.35\textwidth}
    \centering
    \input{tables/poly_ctx}
    \label{table:poly-ctx}
   \end{minipage}\hfill
\end{figure}

We start with a simple polynomial function regression to understand the properties of Meta-Id. In this task, the objective of the models is to identify the context (i.e., the coefficients of the polynomials) and predict the identified functions as show in \cref{fig:poly_overall}.

% \cref{fig:poly_overall} visualize the function regression results.

% \paragraph{Data and baseline} 
We prepare $4^{\text{th}}$ order polynomial datasets by sampling the coefficients from $\mathcal{U}(0.1,2.5)$, and set $N$ and $N'$ as 5 and 15, respectively.\footnote{In the classical setting, at least 5 data points are required to infer the context properly.} The train and test datasets contain 500 and 200 polynomials, respectively. We employ \model{Reptile} \cite{nichol2018first} and \model{ANP} \cite{kim2019attentive} as
the gradient-based and black-box meta-learning method for baselines, respectively. All models, including \model{Meta-Id}, utilize the same multi-layer percetron (MLP) architecture as $f_\theta$ and are trained with data batches for fair comparisons. We provide the details of the model architecture and training scheme in \cref{appendix:poly_detail}. With the polynomial experiments, we discuss the identified properties of \model{Meta-Id} in the following paragraphs.

\paragraph{Does Meta-Id alleviate the ill-conditioned optimization issue?} The predictive performance of the classical parameter identification (\model{Param.Id}) can change significantly depending on the number of context points $N$. However, meta-learning methods can overcome this problem by leveraging the meta-training phase. We validate this by evaluating the predictive performances of the baselines and \model{Meta-Id} with different $N$ on the test dataset. \cref{table:poly-ctx} shows the average mean squared errors (MSE) of the meta-learning methods and \model{Param.Id}. As shown in \cref{table:poly-ctx}, the meta-learning methods generally outperform \model{Param.Id} when $N<5$. Furthermore, \model{Meta-Id} shows the lowest MSE for all $N$. Hence, we can conclude that \model{Meta-Id} alleviates the ill-conditioned optimization issue.

\paragraph{Do $\theta$ and $c$ contain function class and parameter information, respectively?} In the view of the classical parameter identification, the role of $\theta$ and $c$ are to capture a function class and parameterize a specific function from that class, respectively (e.g., $\theta$ expresses the fact that the (meta)-training functions are polynomials and $c$ depicts the coefficients of a specific polynomial). To analyze whether $\theta$ and $c$ accomplish such roles, we train two \model{Meta-Id} models whose parameters are $\theta_1$ and $\theta_2$ from the first (linear) and second (quadratic) order polynomial datasets, respectively. 
We define linearly interpolated parameter $\theta(\tau) \coloneqq(1-\tau)\theta_1+\tau\theta_2$ where $0<\tau<1$. With $\theta(\tau)$ and the context $c \in \mathcal{U}(-\bar c, \bar c)$, we visualize the learned functions $f_{\theta(\tau)}(\cdot; c)$ as shown in \cref{fig:poly-theta-and-c}. From the results, we observe that each $c$ with the given $\theta(\tau)$ parameterizes a function of from the function class (e.g., the red curves are all linear but each of them specific different linear functions). We provide the details of this experiment in Appendix \textcolor{red}{!!}.

% $\theta(\tau)$ from $\theta_1$ to $\theta_2$ with $0<\tau<1$ and then visualize $f_{\theta(\tau)}(\cdot; c)$ where . 

% analyze the role of $\theta$ in \model{Meta-Id}.
\paragraph{Is the target network trick an effective training scheme?} Training \model{Meta-Id} entails solving the bi-level training problem. To understand the effect of the training method (i.e., solving bi-level opt.) on the performance of \model{Meta-Id}, we examine the test MSEs of the different training methods. We compare the test MSE of \model{Meta-Id} trained via (1) target network (\model{Target}), (2) backpropagation-through-optimization (\model{BPTO}), and (3) implicit differentiation of \cref{eq:meta-id-inner} (\model{Implicit}) over the training steps (See \cref{fig:poly-training}). From the results, we confirm that the proposed target network method exhibits stable and better training results. On the contrary, \model{Implicit} fails to converge. This difference can be originated that  \cref{eq:meta-id-inner} generally can not be solved optimally, and the gradient estimation becomes biased \cite{blondel2021efficient, liao2018reviving}. It is also noteworthy that \model{Target} performs stabler and better than \model{BPTO} which is trained in an end-to-end fashion\footnote{All models take the same inner optimization steps, $K=100$; hence this difference is not originated from the inner optimization itself.}. We conjecture this happens because the $f_\theta$ and $f_{\bar \theta}$ are independent during $\theta$ updates and the inferred $c^i$ can be interpreted as noise injected context so that the trained $f_\theta$ becomes robust. Similarly, the relationship between the noise injection and robustness of learned models is studied in \cite{sanchez2020learning, godwin2021very, brandstetter2021message}.


\paragraph{Does the optimization budget affect the predictive performance?} The context inference of \model{Meta-Id} is done by solving \cref{eq:meta-id-inner}. We employ the gradient descent with pre-specified steps $K$ to solve \cref{eq:meta-id-inner}. Hence Meta-Id may have performance variations to $K$. To further analyze this, we train \model{Meta-Id} models with different $K$ and evaluate those on the test dataset. \cref{fig:poly-optstep} visualizes the predictive performance of \model{Meta-Id}s, \model{Reptile}, and \model{ANP}, along with the test time optimization steps. In general, \model{Meta-Id} with higher $K$ performs better at the cost of the increased optimization steps. Additionally, we also observed that the gradient-based methods (e.g., \model{Meta-Id} and \model{Reptile}) could improve the prediction performance by spending more optimization budgets when testing. Nevertheless, \model{Meta-Id} shows a better degree of improvements and asymptotic performances over the optimization steps than \model{Reptile}.

% \cref{fig:poly-training} visualizes the test MSE curves of \model{Meta-Id} trained via (1) target network (\model{Target}), (2) backpropagation-through-optimization (\model{BPTO}), and (3) implicit differentiation of \cref{eq:meta-id-inner} (\model{Implicit}) over the training steps. 



\begin{figure}[t]
   \begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/theta_and_c.pdf}
    \caption{Role of $\theta$ and $c$}
    \label{fig:poly-theta-and-c}
   \end{minipage}\hfill
   \begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/poly_train.pdf}
    \caption{MSE vs. train steps}
    \label{fig:poly-training}
   \end{minipage}\hfill
   \begin{minipage}{0.33\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figs/poly_optsteps_mse.pdf}
    \caption{MSE vs. opt. steps}
    \label{fig:poly-optstep}
   \end{minipage}\hfill
\end{figure}

==> sections/05_2_ts_pred.tex <==
We then evaluate Meta-Id to perform time-series predictions in mass-spring systems which can be described with \textcolor{red}{--} diagram as shown in Figure \textcolor{red}{!!}. Even though the mass-spring is a mathematically simple system, it serves as a fundamental modeling scheme for many engineering problems such as \textcolor{red}{sth. sounds cool + important}\ndref. In this setting, the objective of models is first to infer the physical constants (i.e., the masses and spring constants) from the historical state observations and predicts future state trajectories. 

% \paragraph{Data generation} 
We consider the mass-spring system composed of two distinct masses and three springs without friction. We sample the masses and spring constants from ${\displaystyle {\mathcal {U}}}(0.75,1.25)$ and generate the trajectory of state (i.e., the positions and velocities of masses, 4 dimension) by numerically solving the system equation of mass-spring system for 10 seconds with 0.001 seconds intervals. We set $N$ as 25 (i.e., 0.025 seconds history is used to infer $c$). Training and test dataset are composed of 100 and 50 trajectories, respectively.

% \paragraph{Baseline models} 
We employ variants of \model{GrBAL} \cite{nagabandi2018learning} and \model{ReBAL} \cite{nagabandi2018learning} as the gradient-based and black-box meta-learning baselines. \model{GrBAL} and \model{ReBAL} utilizes MAML \cite{finn2017model} formalism and a RNN encoder to adapt for the specific task, respectively. (i.e., identify the masses and spring constants of the system) Additionally, we employ \model{NoAdapt} which does not explicitly take $c$ as an input of $f_\theta$ to understand the effect of adaptation. For models, including \model{Meta-Id}, we employ the same 1D-convolution network as $f_\theta$ which takes $N$ recent states and $c$ to predict $N$ future states. Please refer \cref{appendix:mass_spring_detail} for the details of network architecture and training of the models.

\paragraph{Numerical results} We assess the predictive performance of \model{Meta.Id} and the baseline models by evaluating the $N$ step prediction (i.e, predicting $N$=25 future states) and the rollout prediction (consecutive 975 future steps) MSE on the test trajectories. As shown in \cref{table:ts-prediction}, \model{Meta-Id} shows significantly lower 1-step and rollout prediction errors, as compared to the baselines. Considering all models utilize the same $f_\theta$ architecture, we can conclude that the optimization-based context identification of Meta-Id is helpful  (or adapt to the specific task) so that the identified context is able to predict near and, also, far future states accurately.

\input{tables/ms_prediction} 

% \begin{figure}[t]
%   \begin{minipage}{0.33\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/theta_and_c.pdf}
%     \caption{Role of $\theta$ and $c$}
%     \label{fig:poly-theta-and-c}
%   \end{minipage}\hfill
%   \begin{minipage}{0.33\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/poly_train.pdf}
%     \caption{MSE vs. train steps}
%     \label{fig:poly-training}
%   \end{minipage}\hfill
%   \begin{minipage}{0.33\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/poly_optsteps_mse.pdf}
%     \caption{MSE vs. opt. steps}
%     \label{fig:poly-optstep}
%   \end{minipage}\hfill
% \end{figure}

==> sections/05_4_traffic.tex <==
\input{tables/traffic}

\ourmodel is devised to solve the meta-learning tasks where each task is assumed to share a common function class and the context $c$ specifies a particular function (i.e., task) as mentioned in \cref{section:intro}. However, the training of \ourmodel can be done without accomplishing the assumptions. In that regard, we hypothesize that \ourmodel learns to generate a ``virtual" context and, by leveraging the learned context, it may improve the performance of general time-series prediction tasks. To validate the hypothesis, we apply \ourmodel to conduct time-series prediction tasks on the real-world traffic dataset.

% , to clearly compare the effect of adaptation

We employ the PeMSD7(M) \cite{yu2017spatio} as our testing dataset. It comprises 228 traffic sensor measurements for the weekdays of May and Jun of 2021 with 5-minute intervals from District 7 of California. The objective is to predict the 15, 30, 45 minute future by considering the recent 60-minute amount of sensor measurements. We employ the spatio-temporal graph convolution network (STGCN) \cite{yu2017spatio} as $f_\theta(\cdot)$ of \model{\ourmodel} and use the same hyperparameter and training setting from \cite{yu2017spatio}, but modified input dimension to accounting for $c$. We employ two types of baselines: (1) non-meta (learned) models, (2) meta-learned models. As non-meta learning baselines, we consider historical average (\model{HA}), linear support vector regression (\model{LSVR}), auto-regressive integrated moving average (\model{ARIMA}), feed-forward neural networks (\model{FNN}), fully connected LSTM (\model{FC-LSTM}), graph convolutional GRU (\model{GCGRU}), STGCN with Chebyshev polynomial approximation (\model{STGCN(Cheb)}), STGCN with the first-order approximation (\model{STGCN(1st)}), and STGCN with Covariance Loss \cite{yoo2021conditional} regularization (\model{STGCN-Cov}). As meta learning baselines, we consider \model{MAML} and \model{Black-box} which employ the same STGCN architecture as $f_\theta$ of \model{\ourmodel}, but utilizes MAML \cite{finn2017model} formalism and STGCN as the history encoder for adaption, respectively. All Meta-learning approaches utilize the recent 60-minute historical observations and their corresponding label to infer context. Note that this context inputs are \textit{only} composed of history; hence we can always use this strategy to construct context inputs. For more training details, please refer Appendix \textcolor{red}{!!}.

\cref{table:pems} summarizes the prediction errors of \model{\ourmodel} and the baselines. From the results, we can find that meta-learning approaches outperform non-meta learning baselines. This might be the effect of using additional data (i.e., the data for the adaption). Among the meta-learning approaches, \model{\ourmodel} shows the leading predictive performances. It is noteworthy that, although \ourmodel is designed to solve meta-learning problems which are assumed to share the same function class, it outperforms general meta-learning methods such as MAML and black-box approaches. To summarize, \ourmodel is possible to extract meaningful ``virtual" context to enhance the predictive performance of models from the data where the real context may not exist.




% As model architecture of \model{\ourmodel} and \model{STGCN(Cheb)} identical but input dimension, we can conclude that utilizing the learned $c$, which is found by solving the inner optimization of meta-id, as an additional input is beneficial to the traffic prediction tasks. In other words, \ourmodel framework is possible to extract meaningful learned context from the set of data where the real context may not exist. 

% For instance, in the following traffic flow prediction tasks, \ourmodel can utilize 

==> tables/ms_prediction.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|ccc|c}
\toprule
& \model{\ourmethod} & \model{GrBAL} & \model{ReBAL} & \model{NoAdapt}  \\
\midrule
$N$-step  & \textbf{0.00006}  & 0.00139  & 0.00050 & 0.00144     \\
Rollout & \textbf{0.17723}  & 0.75690  & 1.84481 & 0.88861     \\
\bottomrule
    \end{tabular}
    \caption{Time-series prediction MSE}
    \label{table:ts-prediction}
\end{table}

==> tables/poly_ctx.tex <==
% \begin{table}
\def\arraystretch{2.0}
\captionof{table}{Prediction MSE}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccc||c}
\toprule
$N$   & \ourmethod & Reptile & ANP & Param. ID  \\
\midrule
1     & \textbf{0.1630}  & 0.1750  & 0.3905 & 0.4989     \\
3     & \textbf{0.0523}  & 0.0958  & 0.0826 & 0.0840     \\
5     & \textbf{0.0268}  & 0.0744  & 0.0495 & 0.0187     \\
10    & \textbf{0.0097}  & 0.0579  & 0.0204 & 0.0000     \\
\bottomrule
\end{tabular}
}

% \end{table}

==> tables/traffic.tex <==
\begin{table}[t]
    % \footnotesize
    \centering
    \caption{PeMSD7(M) results. The performances of the baselines are reproduced from \cite{yu2017spatio}, except \model{STGCN-Cov}.}
    \begin{tabular}{lccc}
        \hline  
        & MAE & MAPE & RMSE \\
        & $(15 / 30 / 45 \mathrm{~min})$ & $(15 / 30 / 45 \mathrm{~min})$ & $(15 / 30 / 45 \mathrm{~min})$ \\
        \cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4}
        \model{HA} & $4.01$ & $10.61$ & $7.2$ \\
        \model{LSVR} & $2.50 / 3.63 / 4.54$ & $5.81 / 8.88 / 11.50$ & $4.55 / 6.67 / 8.28$ \\
        \model{ARIMA} & $5.55 / 5.86 / 6.27$ & $12.92 / 13.94 / 15.20$ & $9.00 / 9.13 / 9.38$ \\
        \model{FNN} & $2.74 / 4.02 / 5.04$ & $6.38 / 9.72 / 12.38$ & $4.75 / 6.98 / 8.58$ \\
        \model{FC-LSTM} & $3.57 / 3.94 / 4.16$ & $8.60 / 9.55 / 10.10$ & $6.20 / 7.03 / 7.51$ \\
        \model{GCGRU} & $2.37 / 3.31 / 4.01$ & $5.54 / 8.06 / 9.99$ & $4.21 / 5.96 / 7.13$ \\
        \hline
        \model{STGCN(Cheb)} & $2.25/3.03/3.57$ & $5.26/7.33/8.69$ & $4.04/5.70/6.77$ \\
        \model{STGCN(1st)} & $2.26/3.09/3.79$ & $5.24/7.39/9.12$ & $4.07/5.77/7.03$ \\
        \model{STGCN-Cov} \cite{yoo2021conditional} & 
        $2.20/2.9 7/3.51$ & $5.14/7.26/8.74$ & $4.02/5.64/6.70$ \\
        \hline
        \model{MAML} & 
        $\textbf{2.17}/2.89/3.21$ &
        $\textbf{5.06}/6.95/7.89$ & $\textbf{3.90}/5.21/\textbf{5.81}$ \\
        \model{Black-box} & 
        $2.24/2.85/3.54$ & $5.19/7.00/8.51$ & $3.96/5.27/6.10$ \\
        \hline
        \model{\ourmethod} & 
        $2.19/\textbf{2.79}/\textbf{3.16}$ &
        $\textbf{5.06}/\textbf{6.81}/\textbf{7.84}$ & $3.93/\textbf{5.17}/5.87$ \\
        \hline
        \end{tabular}
    \label{table:pems}
\end{table}

